Hybrid Digital-Analog Beamforming and MIMO Radar with OTFS Modulation

Motivated by future automotive applications, we study some joint radar target detection and parameter estimation problems where the transmitter, equipped with a mono-static MIMO radar, wishes to detect multiple targets and then estimate their respective parameters, while simultaneously communicating information data using orthogonal time frequency space (OTFS) modulation. Assuming that the number of radio frequency chains is smaller than the number of antennas over the mmWave frequency band, we design hybrid digital-analog beamforming at the radar transmitter adapted to different operating phases. The first scenario considers a wide angular beam in order to perform the target detection and parameter estimation, while multicasting a common message to all possible active users. The second scenario considers narrow angular beams to send information streams individually to the already detected users and simultaneously keep tracking of their respective parameters. Under this setup, we propose an efficient maximum likelihood scheme combined with hybrid beamforming to jointly perform target detection and parameter estimation. Our numerical results demonstrate that the proposed algorithm is able to reliably detect multiple targets with a sufficient number of antennas and achieves the Cram\'er-Rao lower bound for radar parameter estimation such as delay, Doppler and angle-of-arrival (AoA).

==> SimulationResults.tex <==
\section{Numerical Results}\label{sec:Numerical-Results}
\renewcommand{\arraystretch}{1.3}
\begin{table}
	\caption{System parameters}
	\centering
	\begin{tabular}{|c|c|}
		\hline
		$N=6$ & $M=512$ \\ \hline
		$f_c=24.25$ [GHz] & $B=150$ [MHz] \\ \hline
		$v_{\mathrm{res}}\simeq440$ [km/h] & $r_{\mathrm{res}}\simeq1$ [m]\\ \hline
		$v_{\mathrm{max}}=N\cdot v_{\mathrm{res}}$ & $r_{\mathrm{max}}=M\cdot r_{\mathrm{res}}$ \\ \hline
		$\Pav=40$ [mW] & $\sigma_{\mathrm{rcs}}=1$ [m$^2$] \\ \hline
		Noise Figure $=3$ [dB] & Noise PSD = $2\cdot10^{-21}$ [W/Hz] \\ \hline
	\end{tabular}
	\label{tab:System-Parameters}
\end{table}

The number of \ac{RF} chains $\Nrf=8$ is set such that a single equipment is able to jointly track and communicate to $\Nrf$ separately targets (or groups of targets), while $\Nrf\ll\Na$. Table \ref{tab:System-Parameters} provides the system parameters. 

In our simulations, we rely on the following assumptions:
\begin{itemize}
	\item Given the choice of a \ac{mmWave} communication, we assume \ac{LoS} between the \ac{Tx} and the \ac{Rx} (or radar target) \cite{kumari2018ieee,nguyen2017delay}. This is motivated by the fact that any possible scattering component different from the \ac{LoS} generally brings much lower power, given by additional reflections of the echo signal.
	\item Any backscattered power to the radar \ac{Rx} is considered as a possible target. The objective is to sense the surrounding environment, and the differentiation between active targets and obstacles is a post-processing decision. Clearly, in a second phase, communication is established only towards active target (there is no interest to send information to a tree). 
	\item We consider the complete blockage of the signal propagation to the first object hit. This assumption is completely fulfilled in \ac{mmWave} communication scenarios.\footnote{Note that the proposed algorithm could be able to correctly distinguish more targets sharing the same angular direction, if separated in at least one other domain (Doppler or delay) \cite{gaudio2020joint}.} 
\end{itemize}
Note that the aforementioned assumption are shared by many works in literature (see, e.g., \cite{grossi2018opportunisticRadar} and references therein).

% Following the approach of \cite{grossi2018opportunisticRadar}, which follows \cite{rappaport2012propagation,rappaport2015wideband}, 
The radar two-way \ac{PL} is defined as \cite[Chapter 2]{richards2014fundamentals}
\begin{equation}
	\mathrm{PL}=\frac{(4\pi)^3r^{4}}{\lambda^2}\,,
\end{equation}
% such that the standard \ac{PL} (see, e.g., \cite[Chapter 2]{richards2014fundamentals}) formula is obtained for $\eta=2$, while, at \ac{mmWave} at $f_c=24.25$ GHz \cite{braun2014ofdm,sturm2011waveform}, by properly taking into account additional gases absorption effects \cite{rappaport2012propagation}, a more precise formulation of the \ac{PL} requires $\eta=2.5$. 
and the definition of the radar \ac{SNR} becomes 
\begin{equation}
	\mathrm{SNR}=\frac{\lambda^2\sigma_{\mathrm{rcs}}G_\mathrm{Tx}G_\mathrm{Rx}}{\left(4\pi\right)^3r^4}\frac{\Pav}{\sigma_w^2}\,,
\end{equation}
where $\lambda=c/f_c$ is the wavelength, $c$ is the speed of light, $\sigma_{\mathrm{rcs}}$ is the radar cross-section of the target in $\mathrm{m}^2$, $G_\mathrm{Tx}$ and $G_\mathrm{Rx}$ are the antenna gains at the \ac{Tx} and \ac{Rx} respectively, $r$ is the distance between \ac{Tx} and \ac{Rx}, and $\sigma_w^2$ is the variance of the \ac{AWGN} noise with noise \ac{PSD} of $2\cdot10^{-21}$ [W/Hz]. We choose $\sigma_{\mathrm{rcs}}=1$ [m$^2$], while different choices can be found in literature \cite{suzuki2000measurement,kamel2017RCSmodeling}. Note that, while $G_\mathrm{Tx}$ can change with the operational mode, $G_\mathrm{Rx}$ is keep constant (within the angular sector of interest) in order to allow isotropic reception, as already explained. Information about antenna gains, beam patterns, two-way (\ac{Tx} and \ac{Rx}) beamwidth, and more antenna basics (also for mono-static radars) can be found, for instance, in \cite{visser2006array,friedlander2012transmit}.

While two distinct targets in the angle domain can be identified if the angular resolution meets some conditions (depending on the number of antennas, the angular distance between the two targets, and the antenna array properties) \cite{richards2014fundamentals}, a different analysis has to be done for Doppler and delay. In brief, given the parameters listed in Table \ref{tab:System-Parameters}, velocity and range resolutions are
\begin{equation}\label{eq:Radar-Resolution}
v_{\mathrm{res}}=\frac{Bc}{2NMf_c}\ \mathrm{[m/s]}\,,\:\:\:r_{\mathrm{res}}=\frac{c}{2B}\ \mathrm{[m]}\,.
\end{equation}
In order to get a reasonable range resolution, e.g., $<1$ [m], a large bandwidth has to be considered.\footnote{Note that a tradeoff appears. Larger bandwidths mean more precise resolution, but lower theoretical maximum range (with the same $N\times M$ grid). We remark that our algorithm is completely independent of these choices.} Since the velocity resolution is directly proportional to $B$, for a fixed $f_c$, the only way to obtain a lower values is to increase the block size $NM$, leading to a remarkable increase in computational complexity, which could be not affordable. For this reason, we set the system parameters by focusing on a reasonable range resolution (and theoretical maximum range) under a feasible computational complexity. Note that the maximum range could not be achieved if the \ac{PL} brigs the backscattered power below the noise floor. This in turn leads to an unavoidable very large velocity resolution. Note that, given the assumptions taken at the beginning of Section \ref{sec:Numerical-Results}, the problem of targets identifiability appears only in the angular domain, given the total blockage of the signal power within a given direction. However, this only happens at \ac{mmWave}, thus, range and velocity resolutions are reported here for completeness, since the proposed scheme could target lower frequencies, where the aforementioned assumption might not be satisfied. 

\begin{remark}
	The parameters estimation performance of the proposed \ac{ML}-based algorithm strictly depends on the dimension of the block of data sent, i.e., the product $N\cdot M$. Thus, the system parameters of Tab. \ref{tab:System-Parameters} can be easily tuned to achieve the desired levels of radar resolutions (modifying the bandwidth), acquisition time (based on the length of the \ac{OTFS} frame in time), maximum range, etc. Clearly, the \ac{CRLB} changes accordly. Moreover, note that this is also possible thanks to \ac{OTFS} modulation, which is not sensitive to Doppler and delay effects.   
\end{remark}

\begin{remark}
	Radar range and velocity resolutions indicates the minimum necessary targets spacing, in one of the two domain, such that both of them are distinguishable at the radar \ac{Rx}. This has not to be confused and it is not linked to the performance of our \ac{ML}-based detector, which is, indeed, a super-resolution method, able to produce radar parameters estimates with error remarkably lowers w.r.t. the aforementioned resolutions. Thus, there is a huge difference between targets identifiability and estimation performance.
\end{remark}

\begin{figure}
	\centering
	\includegraphics[scale=0.65]{./rangeVelocityAOA_BF_Range.pdf}
	\caption{\ac{Tx} broadcasting a common message. Single target at a different distance within the illuminated angular sector of specified coverage. RMSE performance with associated CRLB and detection performance. $N_a=128$.}
	\label{fig:Detection-Range-Na128}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[scale=0.65]{./rangeVelocityAOA_BF_2Targets.pdf}
	\caption{\ac{Tx} broadcasting a common message. Two target, one fixed at $10$ [m] and the other moving at a different distance (x-axis) within the illuminated $10^\circ$ angular sector. RMSE performance with associated CRLB. Detection performance. $N_a=128$.}
	\label{fig:Detection-Range-Na128-2Targets}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[scale=0.2]{./Fig2Ex.pdf}
	\caption{Example of scenario depicted in Fig. \ref{fig:Detection-Range-Na128-2Targets}. The moving target, in blue, changes its location. A masking effect is related to the fixed target.}
	\label{fig:Ex-Scenario-MovTarget}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[scale=0.63]{./rangeVelocityAOA_BF10_SNR.pdf}
	\caption{\ac{Tx} BF distinct beams towards three different targets. Reception is isotropic, thus AOA estimation is possible (See Fig. ... on the left). Different numbers of antennas. RMSE performance is calculated for one target, while the others are randomly placed and act as interference.}
	\label{fig:BF-Targets}
\end{figure}

\subsection{Simulation Results}
Fig. \ref{fig:Detection-Range-Na128} shows the acquisition performance in terms of \ac{Pd} for a \ac{Tx} broadcasting a common message (see Fig. \ref{fig:Operational-Modes}), while performing estimation of the parameters of interest of the (single) target within an angular sector of different width. First, note that, by considering an angular coverage of $10^\circ$ degrees, the maximum range to correctly identify a target, limited by the \ac{PL} and thus different from he theoretical limit indicated in Table \ref{tab:System-Parameters}, is about $110$ m. For any distance between \ac{Tx} and target, the estimation performance of radar parameters of interest (range, velocity, and \ac{AoA}) follows the corresponding \ac{CRLB}. More in details, note that at the limit range of $110$ m, the \ac{RMSE} for range, velocity, and angle are respectively, $\simeq4\cdot10^{-2}$ [m], $\simeq1.6\cdot10^{1}$ [m/s], $\simeq4\cdot10^{-2}$ [degree$^\circ$]. As expected, given the system parameters, the velocity \ac{RMSE} is quite poor, while the others estimation performance are satisfactory. However, a proper \ac{BF} design towards targets, in a successive tracking/communication phase (as said many times in the body of the paper), could improve the estimation performance maximizing the received \ac{SNR}, as showed in next results. As clearly visible in Fig. \ref{fig:Detection-Range-Na128}, the increase of the angle coverage costs in terms of received backscattered power (less \ac{BF} gain), and the maximum identifiability range remarkably decreases. A tradeoff appears: wider angular sectors allow to explore the environment in less time, but with limited maximum range, while narrower sectors maximize the received power and the maximum target range, at the cost of a time consuming beam sweeping search.  

In Fig. \ref{fig:Detection-Range-Na128-2Targets} the performance of the \ac{SIC} technique presented in Algorithm \ref{alg:Joint-Det-Par-Est} is showed. The scenario considers two targets, one at fixed distance of $10$ [m], the other with moving w.r.t. the x-axis, i.e., from $20$ to $150$ [m] (see Fig. \ref{fig:Ex-Scenario-MovTarget}). Note that the nearest target first interferes with the other, such that the interference term $I_p$ in Algorithm \ref{alg:Joint-Det-Par-Est} is exploited, then completely masks the far away target, such that the \ac{SIC} technique becomes necessary. As clearly visible, the performance in terms of \ac{RMSE} remains the same while considering one or two targets, as a confirmation of the validity of the proposed algorithm. The \ac{SIC} starts fail around $90$ [m], i.e., when the range difference is about $80$ [m], such that the masking effect is not removed efficiently and the far away target is not detected. Finally, the curve flats to $P_d=0.5$, because one target out of two is always correctly detected. Note that the red lines of Fig. \ref{fig:Detection-Range-Na128-2Targets} correspond to the blue ones of Fig. \ref{fig:Detection-Range-Na128}. 

Fig. \ref{fig:BF-Targets} depicts the scenario of Fig. \ref{fig:Operational-Modes} on the left side, i.e., a \ac{Tx} \ac{BF} different beams carrying their own information towards multiple targets.\footnote{Theoretically, targets positions (Doppler-delay-angle plane) are granted by some tracking algorithm which processes the radar information to produce an estimation of the (updated) targets locations. In sight of this, we suppose the target positioned within the 3-dB beamwidth of the antenna beam pattern, and the \ac{AoA} \ac{ML} search is performed within that range.} Since the presence of the target within the illuminated sector is given for granted, detection performance is not shown. In this scenario we consider three different targets within an angular sector of $10^\circ$ degrees, such that the \ac{RMSE} performance is related to the target whose range is indicated on the x-axis, while the other two targets act as interference (exploiting the use of Algorithm \ref{alg:Joint-Det-Par-Est} in all possible configurations). Observing Fig. \ref{fig:BF-Targets}, it is clear that performance depends on the number of antennas used (while $\Nrf=8$ is kept constant), since the \ac{Tx} \ac{BF} gain $G_{\mathrm{Tx}}$ is almost equal to $\Na$, i.e., $G_{\mathrm{Tx}}\simeq\Na$. Thus, a larger antenna array size reflects on better \ac{RMSE} performance, confirmed by the corresponding \ac{CRLB}, and larger maximum detectable range (greater received backscattered power). Moreover, note that a (reversed) ``waterfall'' behavior is shown for range and velocity estimation. This is because, even if the presence of the target is given for granted, low \ac{SNR} values might still lead to a large error during the Doppler-delay \ac{ML} maximization (see Algorithm \ref{alg:Joint-Det-Par-Est}). The waterfall behavior is typical of \ac{ML} estimators and has been extensively analyzed in \cite{gaudio2019effectiveness}. Also note that the \ac{AoA} \ac{RMSE} performance is upper limited by the 3-dB beamwidth of the beam pattern (see, e.g., \cite{friedlander2012transmit,visser2006array}). In fact, as the target position lies within the 3-dB beamwidth, also the \ac{AoA} estimation is limited to that range. As a consequence, the \ac{RMSE} does not exceed a systematic error, indicated as $\epsilon_\mathrm{BW}$, calculated by randomly chosen an \ac{AoA} within the range of possibilities. This behavior could be detectable also for range and velocity estimation errors, but at lower \acp{SNR} values, i.e., for much larger range.  

??? Comment on poor velocity estimation ???


